A Bio-Synthetic Modulator Model for Diffusion-based Molecular Communications

In diffusion-based molecular communication (DMC), one important functionality of a transmitter nano-machine is signal modulation. In particular, the transmitter has to be able to control the release of signaling molecules for modulation of the information bits. An important class of control mechanisms in natural cells for releasing molecules is based on ion channels which are pore-forming proteins across the cell membrane whose opening and closing may be controlled by a gating parameter. In this paper, a modulator for DMC based on ion channels is proposed which controls the rate at which molecules are released from the transmitter by modulating a gating parameter signal. Exploiting the capabilities of the proposed modulator, an on-off keying modulation scheme is introduced and the corresponding average modulated signal, i.e., the average release rate of the molecules from the transmitter, is derived in the Laplace domain. By making a simplifying assumption, a closed-form expression for the average modulated signal in the time domain is obtained which constitutes an upper bound on the total number of released molecules regardless of this assumption. The derived average modulated signal is compared to results obtained with a particle based simulator. The numerical results show that the derived upper bound is tight if the number of ion channels distributed across the transmitter (cell) membrane is small.

==> Fig/ACCUP/AccUpp.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA Upper bound, $N=10^7$\hspace{0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA Upper bound, $N=500$\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA Upper bound, $N=100$\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Accurate analysis, $N=10^7$\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA Accurate analysis, $N=500$\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Accurate analysis, $N=100$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Average number of released molecules, $M(t)$}%
\psfrag{020}[tc][tc]{\matlabtextB Time (sec)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.02$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.04$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.06$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.08$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $200$}%
\psfrag{009}[rc][rc]{\matlabtextC $300$}%
\psfrag{010}[rc][rc]{\matlabtextC $400$}%
\psfrag{011}[rc][rc]{\matlabtextC $500$}%
\psfrag{012}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Fig/PBSACC/PBSACC.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA PBS with drift, $N=10^7$, $dt=10^{-6}$\hspace{0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA PBS without drift, $N=10^7$, $dt=10^{-6}$\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA PBS without drift, $N=10^7$, $dt=10^{-5}$\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Accurate analysis, $N=10^7$\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA Accurate analysis, $N=500$\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Accurate analysis, $N=100$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Average modulated signal, $w(t)$}%
\psfrag{020}[tc][tc]{\matlabtextB Time (sec)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.002$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.004$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.006$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.008$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.01$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{006}[bc][bc]{\matlabtextC $\times10^{5}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{009}[rc][rc]{\matlabtextC $1$}%
\psfrag{010}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{011}[rc][rc]{\matlabtextC $2$}%
\psfrag{012}[rc][rc]{\matlabtextC $2.5$}%
%
%% </ytick>

==> Fig/POsignal/POsig.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA $V_{\rm on}=-200$, $V_{\rm off}=-200$\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA $V_{\rm on}=25$, $V_{\rm off}=-200$\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA $V_{\rm on}=50$, $V_{\rm off}=-200$\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA $V_{\rm on}=200$, $V_{\rm off}=-200$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextB Opening probability}%
\psfrag{025}[tc][tc]{\matlabtextB Time (sec)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.005$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.01$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.015$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.02$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.025$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.03$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.035$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.04$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{019}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>
